A Parameter-Free Adaptive Reflected Gradient Method for Monotone Variational Inequalities

We analyze a one-evaluation-per-iteration method for $\mathrm{VI}(C,B)$ with monotone $L$-Lipschitz $B$: $x_{k+1}=P_C(x_k-\lambda B(u_k))$, $u_k=x_k+\theta_k(x_k-x_{k-1})+\beta_k(x_k-u_{k-1})$, $\theta_k+\beta_k=1$. For constant step and summable filter ($\sum_k\beta_k<\infty$) we prove weak convergence via a Lyapunov function with exact rational dissipation budgets, including Malitsky's reflected gradient method. It is robust to summable operator errors; if $C$ is bounded, the constant-step range reaches $\lambda<(\sqrt2-1)/L$. For unbounded $C$ this reduces to an a priori boundedness statement, certified to $\lambda L=0.387$ by dissipation trading; for affine $B$ on polyhedral $C$, $\dist(x_n,S)\to0$ with $\sum_n\dist^2(x_n,S)<\infty$, strong convergence for bounded $C$, and $R$-linear rates after face identification. The main result is a safeguarded adaptive step-size rule needing no $L$ and no extra evaluations, proved weakly convergent unconditionally: a data-driven Lyapunov weight removes $L$ from the dissipation budgets. For affine $B$ with $C=\mathcal H$, sharpness of $\lambda L=1/\sqrt3$ via a rotation lower bound; the same constant is sharp for unconstrained nonlinear $B$, with convergence for square-summable operator values. Unconditional convergence below $1/(\sqrt3\,L)$ reduces to a marginal-pole absolute-stability statement; the projected case remains open. Under strong monotonicity we prove $R$-linear convergence with explicit contraction, and certify $\Omega(L)$ speedups over constant steps. Numerics confirm the gains.

==> tables.tex <==
\caption{Iterations to relative residual $10^{-6}$ (cap $3\cdot10^5$ evaluations; $*$ = not converged).}\label{tab:iters}
method & P1 & P1b & P2 & P3a & P3b\\
\midrule
EG & 1,491 & 1,512 & 30,996 & 11,567 & 11,567\\
adaEG & 9,945 & 10,219 & 150,000$^*$ & 13,363 & 13,363\\
FBF & 5,167 & 5,240 & 98,079 & 20,259 & 20,259\\
PRG & 8,165 & 8,282 & 148,612 & 24,448 & 24,448\\
PEG & 108,212 & 109,855 & 300,000$^*$ & 154,666 & 154,666\\
ours-const & 30,400 & 30,849 & 300,000$^*$ & 44,226 & 44,226\\
ours, $\varkappa=1/6$ & 9,554 & 8,993 & 245,060 & 15,474 & 15,474\\
ours, $\varkappa=0.3$ & 1,316 & 1,395 & 74,940 & 9,487 & 9,487\\
\bottomrule
\caption{Evaluations of $B$ to relative residual $10^{-6}$ (cap $3\cdot10^5$ evaluations; $*$ = not converged).}\label{tab:evals}
method & P1 & P1b & P2 & P3a & P3b\\
\midrule
EG & 2,982 & 3,024 & 61,992 & 23,134 & 23,134\\
adaEG & 19,890 & 20,438 & 300,000$^*$ & 26,726 & 26,726\\
FBF & 10,334 & 10,480 & 196,158 & 40,518 & 40,518\\
PRG & 8,165 & 8,282 & 148,612 & 24,448 & 24,448\\
PEG & 108,212 & 109,855 & 300,000$^*$ & 154,666 & 154,666\\
ours-const & 30,400 & 30,849 & 300,000$^*$ & 44,226 & 44,226\\
ours, $\varkappa=1/6$ & 9,554 & 8,993 & 245,060 & 15,474 & 15,474\\
ours, $\varkappa=0.3$ & 1,316 & 1,395 & 74,940 & 9,487 & 9,487\\
\bottomrule

